Multi-Modal Lidar Dataset for Benchmarking General-Purpose Localization and Mapping Algorithms

Lidar technology has evolved significantly over the last decade, with higher resolution, better accuracy, and lower cost devices available today. In addition, new scanning modalities and novel sensor technologies have emerged in recent years. Public datasets have enabled benchmarking of algorithms and have set standards for the cutting edge technology. However, existing datasets are not representative of the technological landscape, with only a reduced number of lidars available. This inherently limits the development and comparison of general-purpose algorithms in the evolving landscape. This paper presents a novel multi-modal lidar dataset with sensors showcasing different scanning modalities (spinning and solid-state), sensing technologies, and lidar cameras. The focus of the dataset is on low-drift odometry, with ground truth data available in both indoors and outdoors environment with sub-millimeter accuracy from a motion capture (MOCAP) system. For comparison in longer distances, we also include data recorded in larger spaces indoors and outdoors. The dataset contains point cloud data from spinning lidars and solid-state lidars. Also, it provides range images from high resolution spinning lidars, RGB and depth images from a lidar camera, and inertial data from built-in IMUs. This is, to the best of our knowledge, the lidar dataset with the most variety of sensors and environments where ground truth data is available. This dataset can be widely used in multiple research areas, such as 3D LiDAR simultaneous localization and mapping (SLAM), performance comparison between multi-modal lidars, appearance recognition and loop closure detection. The datasets are available at: https://github.com/TIERS/tiers-lidars-dataset.

==> tex_final/boxplot.tex <==
% This file was created by tikzplotlib v0.9.3.
\begin{tikzpicture}

% \definecolor{color1}{rgb}{1,0.85,0.72}
\definecolor{color1}{rgb}{0.73,0.17,0.03}

\definecolor{color0}{rgb}{0.5,0,1}

\begin{axis}[
    height=\figureheight,
    width=\figurewidth,
    axis line style={white},
    legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
    tick align=outside,
    tick pos=left,
    x grid style={white!69.0196078431373!black},
    xmin=0.5, xmax=2.5,
    xtick style={color=black},
    xtick={1,2},
    xticklabels={LoS-FoV, Baseline},
    y grid style={white!90!black},
    ylabel={Angular separation (rad)},
    ymajorgrids,
    ymin=-0.2, ymax=3.15,
    ytick style={color=black},
    % ytick={-3.14,-1.57,0,1.57,3.14},
    ytick={0,1.57,3.14},
    % yticklabels={-$\pi$,-$\pi/2$,0,$\pi/2$,$\pi$},
    yticklabels={0,$\pi/2$,$\pi$},
    scaled y ticks = false
]
\addplot [black, forget plot]
table {%
1 0.671888665909249
1 0.26519936569698
};
\addplot [black, forget plot]
table {%
1 1.11607447169562
1 1.2639975677668
};
\addplot [black, forget plot]
table {%
0.875 0.26519936569698
1.125 0.26519936569698
};
\addplot [black, forget plot]
table {%
0.875 1.2639975677668
1.125 1.2639975677668
};
\addplot [lightgray, mark=+, mark size=3, mark options={solid}, only marks, forget plot]
table {%
1 0.1688171869247
1 0.00275188045108998
1 0.14367841299196
};
\addplot [black, forget plot]
table {%
2 0.632770822752011
2 0.16415703345617
};
\addplot [black, forget plot]
table {%
2 1.14526621803757
2 1.60324907120309
};
\addplot [black, forget plot]
table {%
1.875 0.16415703345617
2.125 0.16415703345617
};
\addplot [black, forget plot]
table {%
1.875 1.60324907120309
2.125 1.60324907120309
};
\addplot [lightgray, mark=+, mark size=3, mark options={solid}, only marks, forget plot]
table {%
2 0.09727988645249
2 0.0417812914883098
2 1.79833233491784
2 2.03697058211828
2 2.31836279451422
2 2.63389514273772
2 2.96658177569715
2 2.98863399239257
2 2.68512883056327
2 2.41810356514095
2 2.1958462749282
2 2.01983458246078
2 1.87936338617503
2 1.76570675644667
2 1.67241794664869
};
\path [draw=black, fill=magenta, opacity=0.42]
(axis cs:0.75,0.671888665909249)
--(axis cs:1.25,0.671888665909249)
--(axis cs:1.25,1.11607447169562)
--(axis cs:0.75,1.11607447169562)
--(axis cs:0.75,0.671888665909249)
--cycle;
\path [draw=black, fill=cyan, opacity=0.42]
(axis cs:1.75,0.632770822752011)
--(axis cs:2.25,0.632770822752011)
--(axis cs:2.25,1.14526621803757)
--(axis cs:1.75,1.14526621803757)
--(axis cs:1.75,0.632770822752011)
--cycle;
\addplot [thick, black, forget plot]
table {%
0.75 0.791403111994706
1.25 0.791403111994706
};
\addplot [thick, black, forget plot]
table {%
1.75 0.873271293432525
2.25 0.873271293432525
};
\end{axis}

\end{tikzpicture}


==> tex_final/eigenvalue.tex <==
% This file was created by matplotlib2tikz v0.7.6.
\begin{tikzpicture}

\begin{axis}[
    height=\figureheight,
    width=\figurewidth,
    axis background/.style={fill=white!91!black},
    axis line style={white},
    tick align=outside,
    tick pos=left,
    x grid style={white},
    xlabel={Time (s)},
    xmajorgrids,
    xmin=-0.1, xmax=15.1,
    xtick style={color=black},
    y grid style={white},
    ylabel={$\lambda_4$ of $R_{\mathcal{G}}(\textbf{z}^{\text{\tiny UWB}})R_{\mathcal{G}}^T(\textbf{z}^{\text{\tiny UWB}})$},
    ymajorgrids,
    ymin=-0.1, 
    % ymax=3.5,
    ytick style={color=black}
]
\addplot [thin, black, mark=x, mark size=0.6, mark options={solid}]
table {%
0.1 11.0478223601051
0.2 11.1089062641868
0.3 10.3859982821927
0.4 9.61931663340136
0.5 9.19813569412637
0.6 9.69638586396975
0.7 10.4931905068403
0.8 10.0977814659899
0.9 8.44002497143339
1 8.32863196339913
1.1 2.60682619130644
1.2 9.66196288960714
1.3 9.9687020960659
1.4 9.89991523758721
1.5 9.29166948139869
1.6 8.96139104637509
1.7 6.96626961829533
1.8 6.57076403232897
1.9 6.29244430618578
2 5.77946427752031
2.1 5.23507177450167
2.2 4.69495140807464
2.3 4.61511651405434
2.4 4.04625372462173
2.5 4.35924140771734
2.6 4.92711047019344
2.7 5.03295485610579
2.8 4.54812264287655
2.9 4.29984807574317
3 1.99522943460176
3.1 12.7268925704041
3.2 20.1069326555198
3.3 4.58640970046222
3.4 4.09710532413419
3.5 4.44794959432591
3.6 4.66857834555023
3.7 4.87965824715175
3.8 5.32842029356328
3.9 5.85814928335332
4 2.00728317622851
4.1 7.58310314881736
4.2 7.41594208490442
4.3 8.09582519256823
4.4 8.33821860346039
4.5 2.67182377440886
4.6 3.15309051867157
4.7 11.2087942024938
4.8 10.3371171676863
4.9 10.6515648747078
5 11.0080062428054
5.1 11.6150259688559
5.2 12.8009926708249
5.3 12.3553786297615
5.4 4.1091371353406
5.5 14.0698027726783
5.6 14.1229171852082
5.7 14.4436214167263
5.8 4.52360609997891
5.9 14.8826268787659
6 4.11108337157918
6.1 13.9978898042081
6.2 13.3111844294957
6.3 13.4728235271728
6.4 12.6482700875689
6.5 11.9812543508928
6.6 11.5699437748363
6.7 12.285577428244
6.8 12.5883872675783
6.9 13.3498901111666
7 14.0144995355324
7.1 14.4027457948356
7.2 14.9600090172054
7.3 15.5438046231887
7.4 15.4462270770402
7.5 15.5189562481969
7.6 14.9097092419524
7.7 13.4401113564387
7.8 11.149643134103
7.9 11.149643134103
8 10.1791607554798
8.1 8.95000751798872
8.2 8.12220091023381
8.3 7.69580753000498
8.4 7.43827850538947
8.5 6.30577551213096
8.6 6.04045443293383
8.7 6.01111210374776
8.8 6.1103696904144
8.9 5.70476681185807
9 5.49759163030881
9.1 5.60164882068057
9.2 6.45185579536381
9.3 6.84494444081288
9.4 7.10881350585978
9.5 7.7286201865936
9.6 2.49402697862664
9.7 9.27187337170398
9.8 9.49714022845664
9.9 9.49714022845664
10 8.61698388162228
10.1 8.3579486202098
10.2 7.26266534390319
10.3 7.09443453157012
10.4 6.45961347642185
10.5 5.48097497590961
10.6 4.63946056121535
10.7 4.40139444621363
10.8 4.52045706481033
10.9 17.1648376693098
11 16.8288707006427
11.1 0.744138831950934
11.2 0.694431697818767
11.3 16.5273965684771
11.4 0.561621439213322
11.5 16.3453322662306
11.6 0.324408565525903
11.7 0.278050982759657
11.8 1.15740711079917
11.9 0.420761240301872
12 0.476992933965817
12.1 0.527120148587424
12.2 0.526253361686173
12.3 0.528567409154624
12.4 0.530461320045675
12.5 0.539530313562194
12.6 0.724114827896598
12.7 0.724114827896598
12.8 0.725038384638198
12.9 0.80084060013586
13 0.839055814670682
13.1 3.1818675599456
13.2 3.48173084321359
13.3 3.66429652032554
13.4 4.1267809472976
13.5 4.35763289552468
13.6 4.75939319022881
13.7 4.56887210459617
13.8 4.57834357237237
13.9 4.57515312572851
14 4.38051873121881
14.1 17.1383992557708
14.2 3.4409148471087
};
\end{axis}

\end{tikzpicture}

==> tex_final/local.tex <==
% This file was created by matplotlib2tikz v0.7.6.
\begin{tikzpicture}

\definecolor{color1}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color0}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}

\begin{axis}[
    height=\figureheight,
    width=\figurewidth,
    axis background/.style={fill=white!91!black},
    axis line style={white},
    legend cell align={left},
    legend style={draw=white!80.0!black},
    tick align=outside,
    tick pos=left,
    x grid style={white},
    xlabel={x (m)},
    xmajorgrids,
    xmin=-1.375, xmax=4.675,
    xtick style={color=black},
    y grid style={white},
    ylabel={y (m)},
    ymajorgrids,
    ymin=0.000999999999999918, ymax=3.279,
    ytick style={color=black},
    % ylabel style={draw, text width=2.5cm, align=center},% 
]
\addplot [thin, color0, mark=triangle*, mark size=0.42, mark options={solid}]
table {%
2.32 1.9
2.29 1.92
2.24 1.97
2.2 1.99
2.15 2.01
2.09 2.06
2.03 2.05
2 2.11
1.98 2.15
1.97 2.18
1.94 2.26
1.91 2.32
1.85 2.39
1.81 2.46
1.74 2.48
1.68 2.5
1.68 2.57
1.64 2.66
1.64 2.7
1.61 2.75
1.55 2.86
1.51 2.92
1.48 2.9
1.46 2.94
1.43 2.98
1.39 2.98
1.37 3
1.36 3.01
1.34 3.03
1.3 3.05
1.29 3.07
1.3 3.08
1.21 3.1
1.25 3.13
1.21 3.05
1.2 2.99
1.19 3.01
1.25 2.9
1.22 2.85
1.24 2.86
1.29 2.8
1.31 2.82
1.33 2.81
1.33 2.77
1.3 2.77
1.3 2.75
1.3 2.76
1.29 2.72
1.27 2.7
1.27 2.72
1.28 2.7
1.29 2.69
1.27 2.61
1.3 2.58
1.36 2.45
1.41 2.38
1.43 2.32
1.47 2.26
1.5 2.2
1.54 2.13
1.56 2.1
1.59 2.05
1.62 2
1.6 1.98
1.64 1.94
1.69 1.93
1.76 1.89
1.82 1.84
1.88 1.78
1.97 1.76
2.03 1.71
2.1 1.72
2.16 1.66
2.2 1.55
2.22 1.54
2.26 1.52
2.31 1.5
2.37 1.51
2.45 1.5
2.51 1.52
2.6 1.53
2.67 1.48
2.76 1.47
2.84 1.43
2.9 1.4
2.97 1.42
3.03 1.37
3.09 1.31
3.15 1.33
3.24 1.31
3.28 1.34
3.34 1.3
3.41 1.31
3.49 1.34
3.54 1.41
3.65 1.45
3.73 1.5
3.74 1.49
3.79 1.51
3.84 1.52
3.9 1.51
3.94 1.52
3.98 1.58
4.02 1.63
4.02 1.68
4.04 1.71
4.08 1.74
4.12 1.8
4.13 1.84
4.14 1.84
4.16 1.88
4.1 1.94
4.12 2.03
4.15 2.11
4.2 2.17
4.22 2.26
4.2 2.35
4.21 2.48
4.24 2.48
4.24 2.59
4.26 2.6
4.26 2.61
4.27 2.64
4.34 2.65
4.38 2.66
4.37 2.66
4.37 2.72
4.35 2.75
4.36 2.76
4.4 2.75
4.38 2.78
4.37 2.79
4.37 2.79
4.37 2.75
4.38 2.71
4.35 2.7
4.35 2.68
4.36 2.66
4.35 2.65
4.32 2.65
4.27 2.64
4.24 2.63
4.2 2.62
4.16 2.64
4.11 2.61
};
\addlegendentry{DRTLS}
\addplot [thin, color1, mark=square*, mark size=0.42, mark options={solid}]
table {%
1.18 1.6
1.23 1.58
1.27 1.55
1.29 1.49
1.3 1.44
1.33 1.42
1.35 1.37
1.4 1.34
1.45 1.27
1.47 1.15
1.49 1.04
1.51 0.95
1.55 0.88
1.61 0.84
1.66 0.82
1.7 0.73
1.72 0.66
1.76 0.62
1.78 0.57
1.8 0.52
1.82 0.45
1.85 0.4
1.88 0.38
1.9 0.33
1.93 0.3
1.95 0.24
1.97 0.23
1.98 0.21
2 0.19
2.01 0.18
2.03 0.19
2.06 0.21
1.99 0.15
2.01 0.15
2.03 0.15
2.05 0.19
2.05 0.24
2.05 0.23
2.05 0.27
2.04 0.33
2.03 0.38
2.01 0.39
2 0.44
1.98 0.44
1.98 0.46
1.98 0.48
1.98 0.55
1.92 0.54
1.89 0.53
1.94 0.62
1.96 0.66
1.98 0.75
1.95 0.79
1.89 0.83
1.85 0.89
1.79 0.96
1.78 1.06
1.76 1.15
1.71 1.2
1.7 1.28
1.68 1.32
1.65 1.39
1.62 1.42
1.58 1.45
1.53 1.46
1.5 1.5
1.46 1.53
1.41 1.59
1.33 1.62
1.26 1.65
1.24 1.7
1.23 1.73
1.21 1.73
1.21 1.75
1.19 1.78
1.17 1.77
1.11 1.67
1.05 1.69
0.99 1.71
0.91 1.71
0.82 1.73
0.71 1.76
0.58 1.75
0.43 1.76
0.34 1.77
0.24 1.78
0.2 1.82
0.1 1.8
0.0299999999999998 1.8
-0.0700000000000003 1.8
-0.13 1.8
-0.21 1.79
-0.26 1.77
-0.32 1.76
-0.36 1.75
-0.39 1.73
-0.42 1.7
-0.43 1.62
-0.47 1.57
-0.52 1.41
-0.57 1.26
-0.59 1.32
-0.65 1.3
-0.76 1.27
-0.79 1.24
-0.97 1.17
-0.98 1.16
-1.07 1.1
-1.02 1.08
-1.02 1.08
-1.03 1.07
-1.1 1.01
-1.07 0.99
-1.06 0.95
-1.02 0.91
-0.99 0.88
-1.05 0.78
-1.02 0.71
-1.03 0.64
-1.03 0.53
-1.04 0.39
-1.04 0.39
-1.03 0.39
-1.01 0.39
-1 0.4
-0.99 0.39
-1 0.38
-1.03 0.37
-1.02 0.37
-1.01 0.36
-1 0.36
-0.97 0.37
-0.94 0.39
-0.93 0.39
-0.91 0.39
-0.9 0.4
-0.91 0.42
-0.89 0.43
-0.9 0.43
-0.92 0.42
-0.93 0.42
-0.96 0.41
-0.94 0.42
-0.830000000000001 0.47
-0.77 0.5
};
\addlegendentry{Collab.}
\end{axis}

\end{tikzpicture}

==> tex_final/speeds.tex <==
% This file was created by matplotlib2tikz v0.7.6.
\begin{tikzpicture}

% \definecolor{color1}{rgb}{1,0.85,0.72}
\definecolor{color1}{rgb}{0.73,0.17,0.03}

\definecolor{color0}{rgb}{0.5,0,1}
\definecolor{color2}{rgb}{0.12,0.47,0.71}

\begin{axis}[
    height=\figureheight,
    width=\figurewidth,
    % axis line style={white},
    % legend cell align={left},
    % legend style={draw=white!80.0!black},
    % tick align=outside,
    % tick pos=left,
    % x grid style={white!69!black},
    % xlabel={x [m]},
    % xmin=-0.2, xmax=33,
    % xtick style={color=black},
    % y grid style={black!69!white},
    % ylabel={y [m]},
    % % ymin=2.91033051003277, ymax=55.6210530906779,
    % ytick style={color=black}
    axis line style={white},
    legend cell align={left},
    legend style={draw=white!80.0!black},
    tick align=outside,
    tick pos=left,
    % title={Velocity profile 2},
    x grid style={lightgray!92.0261437908!black},
    xlabel={time (s)},
    xmin=-1.54, xmax=32.34,
    xtick style={color=black},
    % y grid style={lightgray!92.0261437908!black},
    y grid style={black!69!white},
    ylabel={velocity ($m/s$)},
    ymin=-2.97500000000028, ymax=7.47500000000007,
    ytick style={color=black}
]
\addplot [semithick, black, forget plot]
table {%
-1.54 7
5249.86 7
};
\addplot [semithick, color0, opacity=0.6]
table {%
0 0
0.2 0.249997990616988
0.4 0.749945747705142
0.6 1.24974884165821
0.8 1.74931086139213
1 2.24853544232569
1.2 2.74732628496889
1.4 2.99652898321118
1.6 3.04762785712171
1.8 3.23541310976603
2 2.9977969125286
2.2 2.99652898321117
2.4 2.99652898321118
2.6 2.99652898321116
2.8 2.99652898321119
3 2.99652898321117
3.2 2.99652898321117
3.4 2.99652898321118
3.6 2.99652898321116
3.8 3.11049995143131
4 3.58300505967476
4.2 4.08300505967478
4.4 4.58300505967477
4.6 5.08300505967477
4.8 5.58300505967478
5 6.04981533041884
5.2 5.82536294644046
5.4 5.32536294644047
5.6 4.82536294644045
5.8 4.32536294644048
6 3.82536294644045
6.2 3.32536294644048
6.4 3.00258157274661
6.6 2.99652898321119
6.8 2.99652898321118
7 2.99652898321115
7.2 2.99652898321117
7.4 2.99652898321118
7.6 2.99652898321119
7.8 2.99652898321116
8 2.99652898321116
8.2 2.99652898321117
8.4 2.99652898321117
8.6 2.99652898321112
8.8 2.99652898321118
9 2.99652898321118
9.2 3.06715983143475
9.4 3.39971652012632
9.6 3.08290423657235
9.8 2.99652898321117
10 2.99652898321116
10.2 2.99652898321118
10.4 2.99652898321116
10.6 2.99684543826593
10.8 3.23588427788814
11 3.73567952159748
11.2 4.23567952159747
11.4 4.41617066685249
11.6 3.93629368891717
11.8 3.43629368891717
12 3.03287111090782
12.2 2.99839845482145
12.4 2.99652898321116
12.6 3.15201731353344
12.8 3.64005358861155
13 4.14005358861156
13.2 4.64005358861155
13.4 5.14005358861155
13.6 5.64005358861155
13.8 5.99793252506095
14 5.60690996152673
14.2 5.10690996152672
14.4 4.60690996152672
14.6 4.10690996152672
14.8 3.60690996152673
15 3.12712623587835
15.2 2.99652898321119
15.4 2.99652898321115
15.6 2.99912947778148
15.8 2.99652898321115
16 3.09413518052218
16.2 3.54954465910907
16.4 3.42971290067485
16.6 3.03038163227313
16.8 2.99652898321117
17 2.99652898321116
17.2 2.99758177916069
17.4 3.01069746463361
17.6 3.29677752586051
17.8 3.05859512248599
18 2.99652898321116
18.2 2.99665796224171
18.4 2.99652898321121
18.6 2.99652898321115
18.8 3.09915362376329
19 3.01750602661567
19.2 2.99800307427055
19.4 2.99652898321115
19.6 2.99652898321116
19.8 3.24180074969657
20 3.74173245954015
20.2 3.81230225120095
20.4 3.31498523581708
20.6 3.00103734202187
20.8 2.99652898321116
21 3.01639250388339
21.2 3.38168910311628
21.4 3.88168910311629
21.6 4.38168910311628
21.8 4.88168910311628
22 5.3816891031163
22.2 5.86613333027675
22.4 5.70530445049856
22.6 5.20530445049856
22.8 4.70530445049855
23 4.20530445049856
23.2 3.70530445049861
23.4 3.20729284398838
23.6 2.99652898321115
23.8 2.99652898321115
24 2.99652898321116
24.2 2.99652898321123
24.4 2.99652898321116
24.6 2.99652898321114
24.8 2.99652898321115
25 2.99652898321116
25.2 2.99652898321124
25.4 2.99652898321117
25.6 2.99652898321118
25.8 2.99652898321114
26 2.99652898321115
26.2 2.99652898321122
26.4 2.99652898321117
26.6 3.21061891971898
26.8 3.70894026673845
27 4.20894026673847
27.2 4.67614402108878
27.4 4.45282995593599
27.6 3.95282995593597
27.8 3.45282995593601
28 3.03950657805612
28.2 2.9965289832112
28.4 2.99652898321115
28.6 2.99652898321117
28.8 2.99652898321115
29 2.99652898321112
29.2 3.03330899685951
29.4 3.43742818552814
29.6 3.83541117103763
29.8 3.48572692475838
30 3.05431477104531
30.2 2.99652898321121
30.4 2.99652898321116
30.6 2.99652898321118
30.8 2.99652898321115
};
% \addlegendentry{velocity}
\addplot [semithick, black, dash pattern=on 1pt off 3pt on 3pt off 3pt, forget plot]
table {%
-1.54 2.5
5249.86 2.5
};
\addplot [semithick, black, dash pattern=on 1pt off 3pt on 3pt off 3pt, forget plot]
table {%
-1.54 -2.5
5249.86 -2.5
};
\addplot [semithick, color0, opacity=0.6, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
0 0
0.2 1.24998995308494
0.4 2.49973878544077
0.6 2.49901546976532
0.8 2.49781009866962
1 2.49612290466781
1.2 2.493954213216
1.4 1.24601349121142
1.6 0.255494369552636
1.8 0.938926263221647
2 -1.18808098618718
2.2 -0.0063396465871457
2.4 4.44089209850063e-14
2.6 -8.43769498715119e-14
2.8 1.48769885299771e-13
3 -1.26565424807268e-13
3.2 -4.44089209850063e-15
3.4 7.32747196252603e-14
3.6 -8.88178419700125e-14
3.8 0.569854841100739
4 2.36252554121726
4.2 2.50000000000007
4.4 2.49999999999994
4.6 2.50000000000003
4.8 2.50000000000003
5 2.33405135372034
5.2 -1.12226191989194
5.4 -2.49999999999994
5.6 -2.50000000000012
5.8 -2.49999999999985
6 -2.50000000000012
6.2 -2.49999999999985
6.4 -1.61390686846938
6.6 -0.0302629476770799
6.8 -6.21724893790088e-14
7 -1.4210854715202e-13
7.2 8.43769498715119e-14
7.4 8.21565038222616e-14
7.6 1.11022302462516e-14
7.8 -1.33226762955019e-13
8 -1.77635683940025e-14
8.2 8.88178419700125e-14
8.4 6.66133814775094e-15
8.6 -2.57571741713036e-13
8.8 3.10862446895044e-13
9 -1.55431223447522e-14
9.2 0.353154241117828
9.4 1.66278344345784
9.6 -1.58406141776984
9.8 -0.431876266805895
10 -4.88498130835069e-14
10.2 7.7715611723761e-14
10.4 -8.65973959207622e-14
10.6 0.00158227527387478
10.8 1.19519419811105
11 2.49897621854668
11.2 2.49999999999997
11.4 0.902455726275102
11.6 -2.39938488967664
11.8 -2.49999999999997
12 -2.01711289004675
12.2 -0.172363280431873
12.4 -0.00934735805144804
12.6 0.77744165161141
12.8 2.44018137539053
13 2.50000000000007
13.2 2.49999999999993
13.4 2.50000000000001
13.6 2.50000000000001
13.8 1.789394682247
14 -1.9551128176711
14.2 -2.50000000000008
14.4 -2.49999999999997
14.6 -2.50000000000001
14.8 -2.49999999999993
15 -2.39891862824192
15.2 -0.652986263335802
15.4 -2.06501482580279e-13
15.6 0.0130024728516531
15.8 -0.0130024728516265
16 0.488030986555155
16.2 2.2770473929344
16.4 -0.599158792171077
16.6 -1.9966563420086
16.8 -0.169263245309805
17 -4.44089209850063e-14
17.2 0.00526397974766279
17.4 0.0655784273645921
17.6 1.4304003061345
17.8 -1.19091201687262
18 -0.310330696374153
18.2 0.000644895152739355
18.4 -0.000644895152484004
18.6 -2.75335310107039e-13
18.8 0.513123202760659
19 -0.408237985738087
19.2 -0.0975147617256034
19.4 -0.00737045529697999
19.6 1.77635683940025e-14
19.8 1.22635883242707
20 2.4996585492179
20.2 0.352848958304006
20.4 -2.48658507691933
20.6 -1.56973946897606
20.8 -0.0225417940535566
21 0.0993176033611509
21.2 1.82648299616443
21.4 2.50000000000005
21.6 2.49999999999996
21.8 2.5
22 2.50000000000009
22.2 2.42222113580228
22.4 -0.804144398890982
22.6 -2.49999999999996
22.8 -2.50000000000005
23 -2.49999999999996
23.2 -2.49999999999978
23.4 -2.49005803255111
23.6 -1.05381930388615
23.8 -1.11022302462516e-14
24 2.44249065417534e-14
24.2 3.79696274421804e-13
24.4 -3.61932706027801e-13
24.6 -1.19904086659517e-13
24.8 7.99360577730113e-14
25 3.99680288865056e-14
25.2 3.90798504668055e-13
25.4 -3.61932706027801e-13
25.6 5.55111512312578e-14
25.8 -1.90958360235527e-13
26 7.99360577730113e-14
26.2 3.39728245535298e-13
26.4 -2.66453525910038e-13
26.6 1.07044968253907
26.8 2.49160673509735
27 2.5000000000001
27.2 2.33601877175154
27.4 -1.11657032576395
27.6 -2.5000000000001
27.8 -2.49999999999982
28 -2.06661688939944
28.2 -0.21488797422458
28.4 -2.55351295663786e-13
28.6 7.32747196252603e-14
28.8 -7.105427357601e-14
29 -1.66533453693773e-13
29.2 0.183900068241953
29.4 2.02059594334316
29.6 1.98991492754744
29.8 -1.74842123139625
30 -2.15706076856537
30.2 -0.288928939170467
30.4 -2.8199664825479e-13
30.6 9.76996261670138e-14
30.8 -1.26565424807268e-13
};
% \addlegendentry{acc}










\addplot [semithick, black, forget plot]
table {%
-1.48 7
4849.96 7
};
\addplot [semithick, olive, opacity=0.5]
table {%
0 0
0.2 0.249997990616985
0.4 0.749945747705142
0.6 1.24974884165821
0.8 1.74931086139214
1 2.24999199033554
1.2 2.75
1.4 3.25
1.6 3.75000000000001
1.8 4.24999999999999
2 4.75000000000001
2.2 5.25
2.4 5.75
2.6 6.25
2.8 6.75
3 7
3.2 7
3.4 6.94352948486449
3.6 6.51236474349221
3.8 6.01236474349222
4 5.51236474349221
4.2 5.01236474349225
4.4 4.51236474349222
4.6 4.01236474349222
4.8 3.51236474349221
5 3.06786391375929
5.2 2.99664600035527
5.4 3.00380423719749
5.6 3.3326757269554
5.8 3.7960320043089
6 3.56195918646887
6.2 3.09678164392809
6.4 2.99652898321118
6.6 2.99652898321118
6.8 2.99652898321116
7 2.99652898321115
7.2 2.99652898321118
7.4 2.99652898321117
7.6 2.99652898321116
7.8 2.99652898321118
8 2.99652898321115
8.2 2.99652898321117
8.4 2.99652898321116
8.6 3.16515851053338
8.8 3.65649387675354
9 4.07142306475919
9.2 3.74401160563305
9.4 3.24404744283737
9.6 2.99652898321117
9.8 2.99652898321117
10 2.99652898321116
10.2 2.99652898321118
10.4 2.99652898321117
10.6 2.99652898321118
10.8 3.22778248619257
11 3.72726695902567
11.2 4.09455031821352
11.4 3.7120647835409
11.6 3.21349812069628
11.8 2.99652898321117
12 2.99652898321117
12.2 2.99652898321119
12.4 2.99652898321115
12.6 2.99652898321118
12.8 2.99652898321116
13 2.99652898321116
13.2 2.99652898321118
13.4 2.99652898321115
13.6 2.9965289832112
13.8 2.99652898321114
14 2.99652898321118
14.2 2.99652898321118
14.4 3.02687135580638
14.6 3.42001777658079
14.8 3.92001777658077
15 4.3692816645779
15.2 4.10147072510205
15.4 3.60147072510204
15.6 3.12324552040318
15.8 3.02666724572319
16 3.41943759215176
16.2 3.91943759215174
16.4 4.41943759215174
16.6 4.91943759215174
16.8 5.41943759215173
17 5.91943759215173
17.2 6.41943759215175
17.4 6.89072849451756
17.6 6.99999999999998
17.8 7.00000000000002
18 6.99999999999998
18.2 6.99999999999999
18.4 7.00000000000002
18.6 6.99999999999999
18.8 6.99999999999998
19 7
19.2 7
19.4 7
19.6 7
19.8 6.99999999999998
20 7
20.2 7.00000000000002
20.4 7
20.6 6.99999999999998
20.8 6.99999999999998
21 6.99999999999998
21.2 7.00000000000006
21.4 7.00000000000002
21.6 6.99999999999991
21.8 7.00000000000002
22 7.00000000000006
22.2 6.99999999999995
22.4 7.00000000000006
22.6 6.99999999999995
22.8 6.99999999999998
23 6.99683858645749
23.2 6.69377355121942
23.4 6.1937735512194
23.6 5.69377355121942
23.8 5.19377355121937
24 4.69377355121939
24.2 4.19377355121937
24.4 3.69377355121939
24.6 3.19691677760812
24.8 2.99652898321118
25 2.99652898321115
25.2 2.99652898321118
25.4 2.9965289832111
25.6 2.99652898321134
25.8 2.99652898321117
26 2.99652898321115
26.2 2.99652898321122
26.4 2.99652898321116
26.6 3.05114119636151
26.8 3.47905941483708
27 3.97905924958806
27.2 3.97848452525603
27.4 3.47848452525602
27.6 3.05087165590215
27.8 2.99652898321114
28 3.02131207381444
28.2 3.40285370892234
28.4 3.36857426073109
28.6 3.01140596485248
28.8 2.99771991539794
29 3.01015908437827
29.2 3.36344964812303
29.4 3.50337650018994
29.6 3.06919093080848
};
% \addlegendentry{velocity}
\addplot [semithick, black, dash pattern=on 1pt off 3pt on 3pt off 3pt, forget plot]
table {%
-1.48 2.5
4849.96 2.5
};
\addplot [semithick, black, dash pattern=on 1pt off 3pt on 3pt off 3pt, forget plot]
table {%
-1.48 -2.5
4849.96 -2.5
};
\addplot [semithick, olive, opacity=0.5, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
0 0
0.2 1.24998995308492
0.4 2.49973878544079
0.6 2.49901546976532
0.8 2.49781009866967
1 2.50340564471699
1.2 2.50004004832232
1.4 2.49999999999998
1.6 2.50000000000004
1.8 2.49999999999992
2 2.50000000000008
2.2 2.49999999999996
2.4 2.50000000000003
2.6 2.49999999999997
2.8 2.50000000000002
3 1.24999999999999
3.2 0
3.4 -0.282352575677542
3.6 -2.15582370686139
3.8 -2.49999999999997
4 -2.50000000000005
4.2 -2.4999999999998
4.4 -2.50000000000016
4.6 -2.49999999999997
4.8 -2.50000000000008
5 -2.22250414866459
5.2 -0.356089567020093
5.4 0.0357911842110781
5.6 1.64435744878956
5.8 2.3167813867675
6 -1.17036408920016
6.2 -2.32588771270388
6.4 -0.501263303584545
6.6 -2.66453525910038e-14
6.8 -6.43929354282591e-14
7 -4.21884749357559e-14
7.2 1.33226762955019e-13
7.4 -5.77315972805081e-14
7.6 -4.44089209850063e-14
7.8 1.13242748511766e-13
8 -1.79856129989275e-13
8.2 9.76996261670138e-14
8.4 -1.11022302462516e-14
8.6 0.843147636611068
8.8 2.45667683110083
9 2.07464594002826
9.2 -1.63705729563071
9.4 -2.49982081397844
9.6 -1.23759229813097
9.8 -6.66133814775094e-15
10 -5.99520433297585e-14
10.2 1.06581410364015e-13
10.4 -5.99520433297585e-14
10.6 6.88338275267597e-14
10.8 1.15626751490693
11 2.4974223641655
11.2 1.83641679593929
11.4 -1.91242767336312
11.6 -2.4928333142231
11.8 -1.08484568742555
12 -2.22044604925031e-14
12.2 1.13242748511766e-13
12.4 -1.97619698383278e-13
12.6 1.68753899743024e-13
12.8 -1.33226762955019e-13
13 1.55431223447522e-14
13.2 1.24344978758018e-13
13.4 -1.77635683940025e-13
13.6 2.68673971959288e-13
13.8 -3.13082892944294e-13
14 1.75415237890775e-13
14.2 0
14.4 0.151711862976016
14.6 1.96573210387208
14.8 2.49999999999986
15 2.24631943998569
15.2 -1.33905469737928
15.4 -2.50000000000003
15.6 -2.39112602349432
15.8 -0.482891373399918
16 1.96385173214281
16.2 2.4999999999999
16.4 2.5
16.6 2.49999999999999
16.8 2.49999999999999
17 2.5
17.2 2.50000000000009
17.4 2.35645451182906
17.6 0.546357527412105
17.8 1.73194791841524e-13
18 -1.73194791841524e-13
18.2 4.44089209850063e-14
18.4 1.33226762955019e-13
18.6 -1.33226762955019e-13
18.8 -4.44089209850063e-14
19 9.32587340685131e-14
19.2 0
19.4 -8.88178419700125e-15
19.6 8.88178419700125e-15
19.8 -9.32587340685131e-14
20 9.32587340685131e-14
20.2 8.43769498715119e-14
20.4 -8.43769498715119e-14
20.6 -9.32587340685131e-14
20.8 0
21 -4.44089209850063e-15
21.2 3.59712259978551e-13
21.4 -1.77635683940025e-13
21.6 -5.28466159721575e-13
21.8 5.28466159721575e-13
22 1.77635683940025e-13
22.2 -5.28466159721575e-13
22.4 5.28466159721575e-13
22.6 -5.32907051820075e-13
22.8 1.77635683940025e-13
23 -0.01580706771247
23.2 -1.51532517619034
23.4 -2.50000000000009
23.6 -2.4999999999999
23.8 -2.50000000000026
24 -2.4999999999999
24.2 -2.50000000000009
24.4 -2.4999999999999
24.6 -2.48428386805635
24.8 -1.0019389719847
25 -1.55431223447522e-13
25.2 1.19904086659517e-13
25.4 -3.97459842815806e-13
25.6 1.21014309684142e-12
25.8 -8.61533067109121e-13
26 -8.88178419700125e-14
26.2 3.37507799486048e-13
26.4 -2.64233079860787e-13
26.6 0.273061065751752
26.8 2.13959109237782
27 2.4999991737549
27.2 -0.00287362166015548
27.4 -2.50000000000001
27.6 -2.13806434676934
27.8 -0.271713363455082
28 0.123915453016499
28.2 1.90770817553953
28.4 -0.171397240956288
28.6 -1.78584147939303
28.8 -0.0684302472727216
29 0.0621958449016446
29.2 1.7664528187238
29.4 0.699634260334578
29.6 -2.1709278469073
};
% \addlegendentry{acc}
\end{axis}

% \begin{axis}[
% axis line style={white},
% axis y line=right,
% tick align=outside,
% x grid style={lightgray!92.0261437908!black},
% xmin=-1.54, xmax=32.34,
% xtick pos=left,
% xtick style={color=black},
% y grid style={lightgray!92.0261437908!black},
% ylabel={acceleration [m/s\^2]},
% ymin=0, ymax=1,
% ytick pos=right,
% ytick style={color=black},
% ytick={0,0.2,0.4,0.6,0.8,1},
% yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
% ]
% \end{axis}
\begin{axis}[
    height=\figureheight,
    width=\figurewidth,
    axis line style={white},
    axis y line=right,
    tick align=outside,
    x grid style={lightgray!92.0261437908!black},
    xmin=-1.54, xmax=32.34,
    xtick pos=left,
    xtick style={color=black},
    % y grid style={lightgray!92.0261437908!black},
    y grid style={black!69!white},
    ylabel={acceleration ($m/s^2$)},
    ymin=0, ymax=1,
    ytick pos=right,
    ytick style={color=black},
    ytick={0,0.2,0.4,0.6,0.8,1},
    yticklabels={0.0,0.2,0.4,0.6,0.8,1.0}
]
\end{axis}

\end{tikzpicture}
